Warped modes in flux compactification of type II b supergravity on the conifold

We examine the Kaluza-Klein theory for warped flux compactifications of type $II\ b $ string theory on a Minkowski spacetime $ M_4$ times a conic Calabi-Yau orientifold $X_6$. The region glued along the internal space directions to the bulk of $X_6$ is modeled by the warped undeformed conifold $\calc _6$. The resulting classical vacum solution of Klebanov-Tseytlin solution, valid at large radial distances from the conic singularity, describes a spacetime asymptotic to $ AdS_5 $ times the conifold compact base $ T^{1,1}$. The metric tensor, axio-dilaton and antisymmetric fields part of the 10-d supergravity multiplet bosonic sector decompose into towers of scalar and tensor fields of fixed mass associated to harmonic modes of $T^{1,1}$ and $M_4$. The warped throat deformations by compactification effects are described by means of AdS/CFT duality. The applications are developed within the hard wall approximation for a truncated $ AdS_5 $ spacetime ending on flat boundaries. Numerical results are presented for the mass spectra and interactions of a selected set of singlet and charged modes and for the interactions of graviton modes with embedded branes. We examine the possibility that an interacting gas of warped massive modes produced after brane-antibrane inflation might reheat the universe and leave cold dark matter relics.

==> revstyle.tex <==
% fichier revstyle.tex 
\hfuzz =1pt
\overfullrule =0pt
\newcounter{subequation}[equation]
\makeatletter \fussy \flushbottom
\def \GUT { grand unified theories }
\def \wrt { with respect to }
\def \cft { conformal field theory }
\def \dof { degrees of freedom }
\def \bef { $\beta -$function }
\def \bet { beta function }
\def \mow { modular weights }
\def \loe { low energy }
\def \km { Kac-Moody }
\def \susy { supersymmetry }
\def \susyq { supersymmetric }
\def \sig { $\sigma -$model }
\def \ws { world sheet }
\def \tres { threshold corrections }
\def \L {\Lambda }
\def \l {\lambda } 
\def \ka {\kappa } 
\def \t {\theta }
\def \vt {\vartheta }
\def \T {\Theta }
\def \vT {\hat {\vartheta } }
\def \a {\alpha }
\def \dh {\partial }
\def \d {\delta }
\def \D {\Delta }
\def \bq {\bar q }
\def \bQ {\bar Q}
\def \g {\gamma }
\def \G {\Gamma }
\def \O {\Omega }
\def \o {\omega }
\def \b {\beta }
\def \S {\Sigma }
\def \s {\sigma }
\def \e {\epsilon }
\def \cc { coupling constant }
\def \ccs {coupling constants }
\def \ph { phenomenology } 
\def \pheny { phenomenologically } 
\def \rhs { right hand side } 
\def \lhs {left  hand side } 
\def \ren { renormalization } 
\def \rge { renormalization group equations}
\def \ud { {1 \over 2} } 
\def \ut { {1 \over 3} } 
\def \td {{3 \over  2 }} 
\def \sm { standard model }
\def \q {\eqno  }
\def \mssm { minimal supersymmetric standard model } 
\def \he  { high energy }
\def \st { string theory }
\def \ft { field theory }
\def \cddd { {\cal D } }
\def \cala { {\cal A } }
\def \calc { {\cal C } }
\def \calp { {\cal P } }
\def \caly { {\cal Y } }
\def \calf { {\cal F } }
\def \calg { {\cal G } }
\def \calq { {\cal Q } }
\def \caln { {\cal N } }
\def \call { {\cal L } }
\def \cale { {\cal E } }
\def \calG { {\cal G } }
\def \calH { {\cal H } }
\def \calk { {\cal K } }
\def \calt { {\Theta } }
\def \calT { {\cal T } }
\def \cald { {\cal D } }
\def \cali { {\cal I } }
\def \calj { {\cal J } }
\def \calb { {\cal B } }
\def \calm { {\cal M } }
\def \calr { {\cal R } }
\def \cals { {\cal S } }
\def \calu { {\cal U } }
\def \calo { {\cal O } }
\def \calz { {\cal z } }
\def \cals { {\cal S } }
\def \calv { {\cal V } }
\def \calx { {\cal X } }
\def \calY { {\cal Y } }
%\def \bea {\begin{equation}}
%\def \eea {\end{equation}}
\def \tchi  {{\tilde \chi }}
\def \Eslash {E \kern-.5em\slash}
\def \epslash {\epsilon \kern-.5em\slash}
\def \pslash {p \kern-.5em\slash}
\def \kslash {k \kern-.5em\slash}
\def \Dslash {D \kern-.5em\slash}
\def \hslash {h \kern-.5em\slash}
\def \dslash {\partial \kern-.5em\slash}
\def \vslash {v \kern-.5em\slash}
\def \Gslash {G \kern-.5em\slash}
\def \Hslash {H \kern-.5em\slash}
\def \Fslash {F \kern-.5em\slash}
\def \oslash {o \kern-.5em\slash}
\def \bull {$\bullet  \quad $}
\def \bfA { {\bf A} }
\def \bfB { {\bf B} }
\def \bfS { {\bf S} }
\def \jmp { Jour. Math. Phys. }
\def \ptp { Prog. Theor. Phys. }
\def \ap {Ann. Phys. (NY) }
\def \z {Z. Phys. } 
\def \pr  { Phys. Rev. }
\def \np { Nucl. Phys. }  
\def \arr { Ann. Rev. Nucl. Sci. } 
\def \ar { Ann. Rev. Nucl. Part. Sci. } 
\def \pp { Phys. Reports } 
\def \je { Sov. Phys. JETP } 
\def \prl { Phys. Rev. Lett. } 
\def \pl { Phys. Lett. }
\def \rmp { Rev. Mod. Phys. } 
\def \nc { Nuovo Cimento }
\def \jnp { Sov. Jour. Nucl. Phys. }
\def\NPB#1#2#3 {{\rm Nucl.~Phys.}  {\bf{B#1}}, {#3} (#2)}
\def\NPA#1#2#3 {{\rm Nucl.~Phys.}  {\bf{A#1}}, {#3} (#2)}
\def\PLB#1#2#3 {{\rm Phys.~Lett.}  {\bf{B#1}}, {#3} (#2)}
\def\PR#1#2#3 {{\rm Phys.~Rep.}  {\bf#1}, {#3} (#2)} 
\def\PRD#1#2#3 {{\rm Phys.~Rev.}  {\bf{D#1}}, {#3} (#2)} 
\def\PRL#1#2#3  {{\rm Phys.~Rev.~Lett.}  {\bf{#1}}, {#3} (#2)} 
\def\ZPC#1#2#3 {{\rm Z.~Phys.}  {\bf C#1}, {#3} (#2)} 
\def\JHEP#1#2#3 {{\rm JHEP} {\bf C#1}, {#3}  (#2)}     
\def\IJMP#1#2#3 {{\rm Int. J. Mod. Phys.}  {\bf A#1}, {#3} (#2)} 
\def\JMP#1#2#3 {{\rm J. Math. Phys.}  {\bf #1}, {#3} (#2)}
\def\PTP#1#2#3 {{\rm Prog. Theor. Phys.}  {\bf{#1}}, {#3} (#2)}
\def\FP#1#2#3  {{\rm  Fortsch. Phys.}  {\bf{#1}}, {#3} (#2)}
\def\CMP#1#2#3  {{\rm Comm. Math. Phys.}  {\bf{#1}}, {#3} (#2)}
\def\RMP#1#2#3  {{\rm Rev.  Mod. Phys.}  {\bf{#1}}, {#3} (#2)}
%%%%%%RICCI PACKAGE %%%%%%%%%%%%%
\def\mysavedown#1{\edef\mysubs{\mysubs#1}}
\def\mysaveup#1{\edef\mysups{\mysups#1}}
\def\mydown#1{{\mytensor}_{\vphantom{\mysubs}#1}}
\def\myup#1{{\mytensor}^{\vphantom{\mysups}#1}}
\def\tensor#1#2{
  #1
  \def\mytensor{\vphantom{#1}}
  \def\mysubs{\relax}
  \def\mysups{\relax}
% Make one pass across indices to determine maximum height.
  \let\down=\mysavedown
  \let\up=\mysaveup
  #2
% Now make a second pass to typeset the sub- & superscripts.
  \let\down=\mydown
  \let\up=\myup
  #2
  }
\def\Alt{\mathop{\hbox{Alt}}\nolimits}
\def\Sym{\mathop{\hbox{Sym}}\nolimits}
\def\Del{\mathop\nabla\nolimits}
\def\grad{\mathop{\hbox{grad}}\nolimits}
\def\div{\mathop{\hbox{div}}\nolimits}
\def\extd{\mathop{d}\nolimits}
\def\Lie{\cal L} 
%% Change this to "\Cal L" for amstex

%\rightline {hep-th/}
%\rightline  {T98/}
%\hoffset-1in
%\voffset-1in
%\if@twoside\oddsidemargin15mm
%\evensidemargin15mm\marginparwidth15mm
%\else\oddsidemargin15mm\evensidemargin15mm\marginparwidth15mm\fi
%\footheight12pt\footskip30pt
%\textwidth 18 cm
%\baselineskip15pt
%\textheight 45\baselineskip
%\makeatletter
%Subequations
\def\thesubequation{\theequation\@alph\c@subequation}
\def\@subeqnnum{{\rm (\thesubequation)}}
\def\slabel#1{\@bsphack\if@filesw {\let\thepage\relax
   \xdef\@gtempa{\write\@auxout{\string
      \newlabel{#1}{{\thesubequation}{\thepage}}}}}\@gtempa
   \if@nobreak \ifvmode\nobreak\fi\fi\fi\@esphack}
\def\subeqnarray{\stepcounter{equation}
\let\@currentlabel=\theequation\global\c@subequation\@ne
\global\@eqnswtrue
\global\@eqcnt\z@\tabskip\@centering\let\\=\@subeqncr
$$\halign to \displaywidth\bgroup\@eqnsel\hskip\@centering
  $\displaystyle\tabskip\z@{##}$&\global\@eqcnt\@ne
  \hskip 2\arraycolsep \hfil${##}$\hfil
  &\global\@eqcnt\tw@ \hskip 2\arraycolsep
  $\displaystyle\tabskip\z@{##}$\hfil
   \tabskip\@centering&\llap{##}\tabskip\z@\cr}
\def\endsubeqnarray{\@@subeqncr\egroup
                     $$\global\@ignoretrue}
\def\@subeqncr{{\ifnum0=`}\fi\@ifstar{\global\@eqpen\@M
    \@ysubeqncr}{\global\@eqpen\interdisplaylinepenalty \@ysubeqncr}}
\def\@ysubeqncr{\@ifnextchar [{\@xsubeqncr}{\@xsubeqncr[\z@]}}
\def\@xsubeqncr[#1]{\ifnum0=`{\fi}\@@subeqncr
   \noalign{\penalty\@eqpen\vskip\jot\vskip #1\relax}}
\def\@@subeqncr{\let\@tempa\relax
    \ifcase\@eqcnt \def\@tempa{& & &}\or \def\@tempa{& &}
      \else \def\@tempa{&}\fi
     \@tempa \if@eqnsw\@subeqnnum\refstepcounter{subequation}\fi
     \global\@eqnswtrue\global\@eqcnt\z@\cr}
\let\@ssubeqncr=\@subeqncr
\@namedef{subeqnarray*}{\def\@subeqncr{\nonumber\@ssubeqncr}\subeqnarray}
\@namedef{endsubeqnarray*}{\global\advance\c@equation\m@ne%
                           \nonumber\endsubeqnarray}


%Number equations by section
\@addtoreset{equation}{section}
\renewcommand{\theequation}{\thesection.\arabic{equation}}
%Other macros
%\newcommand{\bm}{\bibitem}
\newcommand{\be}{\begin{equation}} 
\newcommand{\ee}{\end{equation}} 
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bea}{\begin{eqnarray}} 
\newcommand{\eea}{\end{eqnarray}} 
\newcommand{\bsea}{\begin{subeqnarray}} 
\newcommand{\esea}{\end{subeqnarray}}
\newcommand{\nn}{\nonumber}






